Generating Developable 3D Molecules via Pocket-Conditioned Diffusion and Property-Aware Optimization

Drug discovery and development is time-consuming and resource-intensive, motivating computational approaches such as diffusion models for de novo drug design. Many such models follow the structure-based drug design (SBDD) paradigm, generating molecules to fit a target binding pocket. However, existing diffusion-based SBDD methods typically couple pocket and ligand representation learning, model interactions only at the atom level, and prioritize binding affinity over other developability properties. Here, we introduce conDitar-dev, a conditional diffusion-based SBDD framework for generating ligands with strong binding affinities and favorable ADMET properties. It consists of three modules: msPRL, a pretrained multi-scale pocket representation learning module; conDitar, a pocket-conditioned diffusion model guided by msPRL representations; and paOPT, a generation-time method for optimizing ligand developability. On a newly curated benchmark of human disease targets, conDitar outperforms state-of-the-art SBDD baselines, achieving an average binding score of -8.85 kcal/mol. Across five ADMET properties, conDitar-dev improves performance by up to 73% over conDitar. To further validate the abilities of conDitar-dev to generate developable molecules, we have applied it to two validated druggable targets: programmed death-ligand 1 (PD-L1) and colony-stimulating factor 1 receptor (CSF1R) proteins. Top-ranked generatively designed molecules and their analogs have been experimentally synthesized and biologically tested. Two molecules generated directly by conDitar-dev for PD-L1 exhibited SPR-derived $K_D$ values of 3.49 and 3.75 $\mu$M, respectively. Hit expansion based on conDitar-dev-designed molecules identified selective CSF1R inhibitors with IC$_{50}$ values as low as 200 nM, while also uncovering opportunities for drug repositioning.

==> algorithms/predictor.tex <==
\begin{algorithm}[!h]
    \caption{\predictor for ligand denoising}
    \label{alg:predictor}
    	\textbf{Required Input: $\mol_t$, $\pocketset$} 
    \begin{algorithmic}[1]
        \State $\atomscalar_0 = f(\molatomtype_t, t) $  

        \State $\atomvec_0 = \molatompos_t $
        \State $\messatomscalar_0 = f(\atomscalar_0) $
        \State $\messatomvec_0 = f(\atomvec_0) $
        \For{layer $l=1$ to $L$}
            \State $\pcscalar_l, \pcvec_l, \rcscalar_l, \rcvec_l = f(\molatompos_t, \atomscalar_{l-1}, \atomvec_{l-1}, \pocketatompos, \pascalar, \pavec)$ \Comment{learn pocket-ligand interaction (equation \ref{eqn:pc_embed} to \ref{eqn:pil:attn})}
            \State $\messatomscalar_{l}, \messatomvec_{l} = f(\molatompos_t, \atomscalar_{l-1}, \atomvec_{l-1}, \messatomscalar_{l-1}, \messatomvec_{l-1})$  \Comment{learn intra-ligand interaction (equation \ref{eqn:mess:diff_gvp} to \ref{eqn:bond_type})}
            \State $ \atomscalar_l, \atomvec_l = f( \atomscalar_{l-1}, \atomvec_{l-1}, \messatomscalar_{l}, \messatomvec_{l}, \pocketatompos, \pocketatomtype, \pcscalar_l, \pcvec_l, \rcscalar_l, \rcvec_l)$ \Comment{fuse different interactions (equation \ref{eqn:plp:gvp} and \ref{eqn:plp:concat})}
        \EndFor
        \State $\tilde{\molatomtype}_{0,t} = f(\atomscalar_L)$ \Comment{estimate atom types of clean ligand (equation \ref{eqn:pred:pred})}
        \State $\tilde{\molatompos}_{0,t} = \molatompos_{0,t} + \atomvec_L$ \Comment{denoise on atom positions (equation \ref{eqn:pred:pred})}
        \State \Return $(\tilde{\molatompos}_{0,t}, \tilde{\molatomtype}_{0,t})$
    \end{algorithmic}
\end{algorithm}
